SBNet: Sparse Blocks Network for Fast Inference

Conventional deep convolutional neural networks (CNNs) apply convolution operators uniformly in space across all feature maps for hundreds of layers - this incurs a high computational cost for real-time applications. For many problems such as object detection and semantic segmentation, we are able to obtain a low-cost computation mask, either from a priori problem knowledge, or from a low-resolution segmentation network. We show that such computation masks can be used to reduce computation in the high-resolution main network. Variants of sparse activation CNNs have previously been explored on small-scale tasks and showed no degradation in terms of object classification accuracy, but often measured gains in terms of theoretical FLOPs without realizing a practical speed-up when compared to highly optimized dense convolution implementations. In this work, we leverage the sparsity structure of computation masks and propose a novel tiling-based sparse convolution algorithm. We verified the effectiveness of our sparse CNN on LiDAR-based 3D object detection, and we report significant wall-clock speed-ups compared to dense convolution without noticeable loss of accuracy.

==> sections/additional_results.tex <==
% !TEX root = ../supplementary.tex
\section{Additional results}

In the main paper, only conv2-conv5 layers were in sparse mode, and the initial convolution,
upsampling, and output layers were still in dense mode. Here, we converted all of the layers to
sparse mode and retrained the sparse network. We provide the speedup and detection accuracy in
Table~\ref{tab:atg4d}. Full sparse networks have much higher average speedup due to the elimination
of all dense layers, while maintaining similar detection accuracy compared to partial sparse
networks. Average overall timings are reported in Table~\ref{tab:mask_overhead}. The full sparse
network with PSP mask reduces the average timing by another 7ms (34.8ms vs. 27.2ms). We also update
the speedup plot in Figure~\ref{fig:full_speedup}.

\begin{table}
\centering
\caption{Speed-up \& detection accuracy of SBNet on the ATG4D dataset. mAP at 70\% IoU.}
\label{tab:atg4d}
\resizebox{0.49\textwidth}{!}{
\begin{small}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Model       & Sparse        & Train Loss &  Sparsity      & Avg. Speed-up    & mAP         \\
\hline 
Dense       & N/A           & No Mask    &  0\%           & 1.0$\times$      & 74.1        \\  
Dense       & N/A           & Road Mask  &  0\%           & 1.0$\times$      & 75.2        \\
SBNet +Road & conv2-5       & Road Mask  & 75\%           & 1.88$\times$     & \bf{77.2}   \\
SBNet +PSP  & conv2-5       & PSP Mask   & 90\%           & 2.41$\times$     & 73.7        \\
\hline
SBNet +Road & Full          & Road Mask  & 75\%           & 2.03$\times$     & 77.0        \\
SBNet +PSP  & Full          & PSP Mask   & 90\%           & \bf{3.08$\times$}& 73.8        \\
\hline
\end{tabular}
\end{small}
}
\end{table}

\begin{table}
\centering
\caption{Overall network average single forward pass timing and mask network overhead}
\label{tab:mask_overhead}
\begin{small}
\begin{tabular}{|c|c|c|c|}
\hline
Network        & Sparse     & Resolution      & Time (ms)  \\
\hline
Dense          & N/A        & $800\times1408$ & 83.9       \\
\hline
SBNet +Road    & conv2-5  & $800\times1408$ & 44.6       \\
SBNet +PSP     & conv2-5  & $800\times1408$ & 34.8       \\
\hline
SBNet +Road    & Full       & $800\times1408$ & 41.3       \\
SBNet +PSP     & Full       & $800\times1408$ & 27.2       \\
\hline
\hline
PSPNet         & N/A        & $100\times176$  & 3.2        \\
\hline
\end{tabular}
\end{small}
\end{table}


\begin{figure}
\centering
\includegraphics[width=0.9\columnwidth,trim={-1.0cm 0cm 0.0cm 0cm}, clip]{figures/full_speedup_fullsparse_fig.pdf}
\caption{
Full detector network speed-ups for using road map and predicted masks.
Individual frames are plotted as scatter points and an average speed-up in each sparsity level is
plotted with standard deviation.
}
\label{fig:full_speedup}
\end{figure}


==> sections/measurement_details.tex <==
% !TEX root = ../supplementary.tex
\section{Measurement details}

\paragraph{Layerwise timing} For layer-wise experiments we first warm up the computation for 15
times then run the layer for another 15 times, and report the average timing/speedup. We used
cudaEventRecord and cudaEventElapsedTime CUDA runtime API wrapped in TensorFlow custom ops and
inserted into the TensorFlow graph in the beginning and the end of the network. This excludes the
unnecessary TensorFlow session overhead that would not be present in a properly engineered
production inference system.

\paragraph{Full network timing} One of the technical issues we ran into during gathering timings is
that for any specific set of convolution layer parameters (N,C,H,W) either TensorFlow or cuDNN
internally run the  auto-tuner, sweeping over all available convolution algorithms (such as FFT,
Winograd, implicit GEMM etc), picking the fastest one and saving it for subsequent calls. Because
our algorithm often produces a unique new batch size for a given sparsity of the input, we often
observed the autotuner run in the middle of the inference session even after the first image had
gone through the network. Eventually the time settled, however our timings were reported using a
second run of the inference session for the same inputs. 
% A proper technical solution could involve
% either adjusting the autotuner heuristics or rounding up the batch size for sparse convolution
% blocks for autotuning purposes.


==> sections/model_details.tex <==
% !TEX root = ../supplementary.tex
%=================== detector net architect ================
\begin{figure}[t]
\begin{center}
   \includegraphics[width=0.95\linewidth]{./figures/network_architecture_fig.pdf}
\end{center}
   \caption{The network architecture of the detector}
\label{fig:network_architect}
\end{figure}
%==============================================================

\section{Model details} We provide model details in Table~\ref{tab:table_details} and illustrate the
network architecture in Figure~\ref{fig:network_architect}. We first pass the inputs through 2
convolution layers (without intermediate non-linearity or batch-normalization), followed by 4 stages
of the residual network. Downsampling is done by stride 2 convolutions in the first residual unit of
each stage. In the upsample stage, the feature map is upsampled by a factor of 2 via deconvolution,
added with the corresponding feature maps in the backbone network, with an 1x1 convolution to match
the dimensionality. The network has two output branches, one for object classification and one for
object localization. Each branch has 4 convolution layers. The classification branch outputs 1
channel of score map followed by a sigmoid activation function, while the localization branch
outputs 6 channels of geometry information $\{\cos(\theta), \sin(\theta), \log(dx), \log(dy),
\log(w), \log(l)\}$ without non-linearity. The 6 dimensions of the geometry information encode the
heading angle $\theta$ of the vehicle as $\textrm{arctan2}(\sin(\theta), \cos(\theta))$, the
location offset from the vehicle center to the pixel ($dx$, $dy$), and the size of the vehicle ($w$,
$l$) from a bird's eye view.

During inference time, only those locations whose scores are above the threshold $\gamma$ (we set
$\gamma$ to 0.3 empirically) are decoded into detections. Non-maximum suppression (NMS) is used to
get the final detections.

\begin{table}
\centering
\caption{SBNet based fully convolutional LiDAR detector details}
\label{tab:table_details}
\resizebox{0.49\textwidth}{!}{
\begin{small}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Stage         & Input        & \# Layers& Type       &Kernel size& \# Hidden Units         \\
\hline
conv-1        & input        & 2          & Conv       &3$\times$3 & 800$\times$1408$\times$33 \\
\hline
conv-2        & conv-1       & 3          & Residual   &1$\times$1-3$\times$3-1$\times$1 & 400$\times$704$\times$96  \\
conv-3        & conv-2       & 6          & Residual   &1$\times$1-3$\times$3-1$\times$1 & 200$\times$352$\times$192 \\
conv-4        & conv-3       & 6          & Residual   &1$\times$1-3$\times$3-1$\times$1 & 100$\times$176$\times$256 \\
conv-5        & conv-4       & 3          & Residual   &1$\times$1-3$\times$3-1$\times$1 & 50$\times$88$\times$384   \\
\hline
conv-6        & conv-5       & 1          & Conv       &1$\times$1&  50$\times$88$\times$196   \\
upsample-7    & conv-6, conv-4 & 1        & Deconv+Conv&3$\times$3, 1$\times$1&  100$\times$176$\times$128 \\
upsample-8    & upsample-7, conv-3 & 1    & Deconv+Conv&3$\times$3, 1$\times$1&  200$\times$352$\times$96  \\
\hline
output-cls-1  & upsample-8   & 4          & Conv       &3$\times$3&   200$\times$352$\times$64  \\
output-cls-2  & output-cls-1 & 1          & Conv       &3$\times$3&   200$\times$352$\times$1   \\
\hline
output-reg-1  & upsample-8   & 4          & Conv       &3$\times$3&   200$\times$352$\times$64  \\
output-reg-2  & output-reg-1 & 1          & Conv       &3$\times$3&   200$\times$352$\times$6  \\
\hline
\end{tabular}
\end{small}
}
\end{table}

% %=================== detector net architect ================
% \begin{figure}[t]
% \begin{center}
%    \includegraphics[width=0.95\linewidth]{./figures/network_architecture_fig.pdf}
% \end{center}
%    \caption{The network architecture of the detector.}
% \label{fig:network_architect}
% \end{figure}
% %==============================================================



==> sections/pascal.tex <==

% \subsection{Camera object detection} In applications such as camera object detection, the
% computation mask can be obtained using a semantic segmentation network to predict the foreground heatmap.

% We comprehensively evaluate our method on the PASCAL VOC 2007 detection benchmark \cite{pascal},
% which consists of about 5k trainval images and 5k test images over 20 object categories.

% \subsubsection{Model}
% \AP{We could use better consistency in use/used past/present tense across the entire paper - which one is the right way?}
% We use an off-the-shelf Faster-RCNN detector model with a ResNet-101 trunk. We use two variants of the PSP network \cite{psp} to predict foreground segmentation mask. We designed two models,
% the smaller one designated as "PSP-Lite" which has a much lower compute overhead compared to the original PSP network.

% The mask is dilated and binarized, and applied at different resolution stages of ResNet-101, from conv2 to conv4. During training, we jointly finetune the foreground network, and the mask is directly applied with dense multiplication to be end-to-end differentiable.

% \begin{table*}
% \centering
% \caption{PASCAL detection accuracy on Car3D dataset.}
% \label{tab:pascal}
% \resizebox{1.0\textwidth}{!}{
% \begin{small}
% \begin{tabular}{c|c|c|cccccccccccccccccccc}
% Model          & Speed-up   & mAP  & aero & bike & bird & boat & bottle & bus & car & cat & chair & cow & table & dog & horse & mbike & person & plant & sheep & sofa & train & tv \\
% \hline 
% Dense       & 1.0$\times$& 73.3 & 76.6 & 78.7 & 76.6 & 59.9 & 56.2 & 78.3 & 85.2 & 86.5 & 52.2 & 82.3 & 66.9 & 87.3 & 85.2 & 77.9 & 77.8 & 44.3 & 74.6 & 75.2 & 76.7 & 67.9 \\ 
% \hline
% SBNet no FT   & TBD      & 47.6 & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD& TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD \\
% SBNet +PSP FT& TBD    & 71.7 & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD& TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD \\
% SBNet +PSPLite FT& TBD    & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD& TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD \\
% \end{tabular}
% \end{small}
% }
% \MR{Maybe add ablation studies of adding sparse at various level of resolution.}
% \end{table*}

% \begin{table}
% \centering
% \caption{Mask network computation overhead}
% \label{tab:mask_overhead}
% \begin{small}
% \begin{tabular}{c|c|c}
% Network         & Resolution      & Time (ms)  \\
% \hline
% Dense Detector  & $600\times1000$ & 125        \\
% Sparse Detector & $600\times1000$ &            \\
% \hline
% Mask Net        & $150\times150$  & 12.6       \\
% Mask Net Small  & $100\times100$  & 11.1       \\
% \end{tabular}
% \end{small}
% \end{table}

% \subsubsection{Results and Discussion} Table~\ref{tab:pascal} show detection accuracy mAP@0.5 on
% all 20 object classes. SBNet shows a mild accuracy decrease of 2 points compared to dense
% network, while achieving speed-up of xx. We further investigated the computation overhead of the mask
% network in Table~\ref{tab:mask_overhead}. While full segmentation network has larger computation
% overhead, the lightweight network has much less overhead while achieving similar detection
% accuracy.


==> sections/training_details.tex <==
% !TEX root = ../supplementary.tex
\section{Training details}

The loss function of our detector is a combination of the focal loss (FL) \cite{focal} on the
classification sub-task and the smooth $\ell_1$ loss (Huber loss) on the regression sub-task. We sum
the classification loss over all samples and only compute the regression loss on positive samples.
Both classification and regression losses are averaged by the number of positive samples.

\begin{equation}
\begin{aligned}
    L_\text{total} & = \textrm{FL}(p, y) + \textrm{Huber}(q - g),
\end{aligned}
\end{equation}
where
\begin{align}
    \textrm{FL}(p, y) &= 
    \begin{cases}
      -0.25(1-p)^2\text{log} (p)& \text{if } y = 1,\\
      -0.25p^2\text{log} (1-p)& \text{if } y = 0,
    \end{cases}\\
      \textrm{Huber}(x) &=
  \begin{cases}
    0.5x^2& \text{if } |x| < 1,\\
    |x| - 0.5& \text{otherwise}.
  \end{cases}
\end{align}
Our network is trained using SGD with momentum optimizer with initial learning rate 1e-3 and
momentum 0.9 for a total of 120K steps. The learning rate is multiplied by 0.1 at 100K steps. We
initialize the weights of the network randomly following Xavier initialization \cite{xavier}. 
We use a mini-batch size of 2.


==> sections/video.tex <==
% !TEX root = ../supplementary.tex
\section{SBNet visualization}
Please see our attached supplementary video for a dynamic visualization of the SBNet-based
LiDAR detector in action.
\begin{figure}
\centering
\includegraphics[width=0.99\columnwidth,trim={0cm 0cm 0cm 0cm}, clip]{figures/vid_screenshot.png}
\caption{A screenshot of our video, comparing Dense, SBNet+Road, and SBNet+PSP.}
\label{fig:video}
\end{figure}

